CrowdPlanner: A Crowd-Based Route Recommendation System

CrowdPlanner -- a novel crowd-based route recommendation system has been developed, which requests human workers to evaluate candidates routes recommended by different sources and methods, and determine the best route based on the feedbacks of these workers. Our system addresses two critical issues in its core components: a) task generation component generates a series of informative and concise questions with optimized ordering for a given candidate route set so that workers feel comfortable and easy to answer; and b) worker selection component utilizes a set of selection criteria and an efficient algorithm to find the most eligible workers to answer the questions with high accuracy.

==> 1 IEEE_Paper_LaTeX_Template_LETTER_V2 20130719/abstract.tex <==

\begin{abstract}
As travel is taking more significant part in our life, route recommendation service becomes a big business and attracts many major players in IT industry. Given a user specified origin and destination, a route recommendation service aims to provide users the   routes  with the best travelling experience according to criteria such as travelling distance, travelling time, traffic condition, etc. However, previous research shows that even the routes recommended by the big-thumb service providers can deviate significantly from the routes travelled by experienced drivers. It means travellers' preferences on route selection are influenced by many latent and dynamic factors that are hard to be modelled exactly with pre-defined formulas.  In this work we approach this challenging problem with a completely different perspective -- leveraging crowds' knowledge to improve the recommendation quality. In this light, CrowdPlanner -- a novel crowd-based route recommendation system has been developed, which requests human workers to evaluate candidates routes recommended by different sources and methods, and determine the best route based on the feedbacks of these workers. Our system addresses two critical issues in its core components: a) task generation component generates a series of informative and concise questions with optimized ordering for a given candidate route set so that workers feel comfortable and easy to answer; and b) worker selection component utilizes a set of selection criteria and an efficient algorithm to find the most eligible workers to answer the questions with high accuracy. 

%Route recommendation is one of the most widely used spatial services nowadays. 
%A pleasant drive is the basis of a pleasant trip. 
%Many big thumb IT companies have provided many successful route recommendation services. 
%Users follow these services' navigation guide with their absolute trust, but some experiments have shown that the routes recommended by services are always different from experienced drivers' preference. 
%The phenomenon is difficult to find out since the driver's preference is infected by many latent factors, which can hardly predefine. 
%Though there are many popular route detecting algorithms by mining historical trajectories, it is still not easy to get the drivers' most prefer route due the sparse of trajectories and the disagreement among many algorithms. 
%In this paper, we pioneer a systematic approach to evaluate the recommended levels of routes provided by web services and popular routes mining algorithms. 
%Specifically, we build the CrowdPlanner system to give users the verified best routes and allow computers together with crowds to evaluate routes effectively and efficiently. 
%When a route recommendation request is given by end users, the system will generate the candidate route from different providers, i.e., web services and popular route mining algorithms, and evaluate these candidate routes using the in-hand information.
%If the in-hand information is not enough to support the system to give high confidence evaluation, the system will invoke the crowds to evaluate them. 
%We propose an automatic evaluating route task generating algorithm, which ensures the final evaluating quality and reduces the workload of crowds in a large degree. 
%Also, we propose a novel worker selecting method which can find the most eligible workers, who have good knowledge of the task, can response in a tolerable time and so on, of a certain task. 
%Finally, we conduct extensive experiments involving a lot of volunteers and using real trajectory datasets to demonstrate the effectiveness and efficiency of the proposed CrowdPlanner system. 
\end{abstract}

% NOTE keywords are not used for conference papers so do not populate them
\begin{keywords}
Crowdsourcing
\end{keywords}


==> 1 IEEE_Paper_LaTeX_Template_LETTER_V2 20130719/conclusions.tex <==
\section{Conclusions}\label{sec:conclusion}

In this paper we have taken an important step towards evaluating recommended routes from different providers, web services and popular routes mining algorithms, to provide users the verified best routes. 
After studying the difference between web service recommended routes and popular routes mined from historical trajectories, we have proposed a system CrowdPlanner which give users the verified best routes and allow computers together with crowds to evaluate routes effectively and efficiently. 
We use many components to reduce the time cost and manpower cost of the route evaluating procedure, such as,  truth reusing, landmark selecting and worker selecting, where in this paper we details the human evaluating related part. 
Landmark selecting automatically generates an identifiable set of landmarks with the highest mean significance. 
Worker selecting finds the top-k most eligible workers who have good knowledge of the task. 
Extensive experiments have been conducted involving a lot of volunteers and using a real trajectory dataset. 
We have demonstrated that the CrowdPlanner system can always give users the best routes. 
The MFP (Mining Frequent Path) has the highest possibility to give the best route. 
The ideas from this work open a new direction for future research, such as quality control of popular route mining algorithms, and mining latent factor which may affect drivers' driving routes.

==> 1 IEEE_Paper_LaTeX_Template_LETTER_V2 20130719/findtargetworker.tex <==


\section{Worker Selection}\label{sec:targetworker}
Some Crowdsourcing platforms such as AMT and CrowdFlower give workers the freedom to choose any questions.
However this may cause some problems, for example, many workers choose to answer a same question while some other questions are not picked by anyone, workers have to view all the questions before they choose,  workers may answer questions that they are not familiar with. 
CrowdPlanner avoids these problems by  designing a dedicated component to assign each task to a set of eligible workers.
In order to judge whether a worker is eligible for a task, many aspects of the worker have to be taken into consideration, i.e., number of outstanding tasks, worker's response time and familiarity with a certain area.
First, since each worker may have many outstanding tasks, in order to balance the workload and reduce the response time, we use a threshold $\eta_{\#q}$ to restrict the maximum number of tasks of each worker.
Second, each user of CrowdPlanner can specify the longest time delay she allows to get an answer, so this task will not be assigned to workers who have high probability not to accomplish the task before the due time.
Last, a recommended route will have high confidence to be correct if assigned workers are very familiar with this area. 
Again, the worker's familiarity with respect to a certain area can also be affected by several factors, such as whether the worker lives around the area, whether the worker has answered questions relating to this area correctly in the past, etc. 
In summary, an eligible worker should meet three conditions: 1. has quota to answer the question; 2. has high probability to answer a question before due time;  3. has relatively high familiarity level with the query regions.

%In this section, we will formally quantify the familiar level of a region, define the top-k eligible query and describe detailed processing of the query.

\subsection{Response Time} \label{set:Response Time}

Each task has a user-specified response time, with which an answer must be returned. 
We assume the probability of the response time $t$ of a worker follows an exponential distribution~\cite{Doe:2009:exponentialdistribution}, i.e., $f(t; \lambda) =\lambda \exp^{-\lambda t}$, which is standard assumption in estimating worker's response time.
%The probability of a worker to respond a task within time $t$ is calculated by $\Pr (rt\le t)$.
The cumulative distribution function of $f(t;\lambda)$ is  $F(t;\lambda)= 1-\exp ^{-\lambda t}$. If the probability of a worker to respond a task within time $\overline t$, represented by $F (\overline t; \lambda)$, is less than the threshold $\eta_{time}$, we will not assign the task to him.

\subsection{Worker's Familiarity Score}


%Due people's different living regions and visiting places, people have different knowledge of places that they are more
%Different people living in different areas and visit different places, %which leads them to have different
%Whether a worker has a good knowledge to answer a question is  answer a task
People usually have the best knowledge for areas where they live or travel about frequently. %, while it is common that people have less knowledge of lives in other regions of the same city, th have less knowledge of
%People' knowledge of a certain thing
%In order to improve the quality of recommended routes, a question should be answered by people who have best knowledge of it.
%However, the knowledge of a certain region of a person is hard to measure.
In CrowdPlanner, we develop a familiarity score $f_w^l$ to estimate the knowledge of a worker $w$ about a landmark $l$. 
$f_w^l$ is mainly affected by two factors: (1) worker's profile information, including her home address, work place and familiar suburbs, which can be collected during her registration to the system, and (2) history of worker's tasks around this area.
$f_w^l$ of landmark is defined as:

\begin{align*}
f_w^l =& \alpha\cdot\exp{\{
-(d(l,p_{home})+d(l,p_{work})+d(l, p_{fr})\}} \\
&+(1-\alpha)\cdot(\#correct+\beta\cdot \#wrong)
\end{align*}


where $\alpha$ is a smoothing variable, $d(l,p_{*})$ is the distance between $l$ and $p_{*}$, $\#correct$ is the number of correctly answered question of $l$, $\#wrong$ is the number of incorrectly answered question of $l$, and $\beta$ is a constant less than $1$, which measures the gain of a wrong answer.
Notably, since the knowledge of a far away region can hardly influence the knowledge here and in order to simplify the computation of $f_w^l$, we assign $+\infty$ to $d(l,x)$ if $d(l,p_{*})$ is bigger than a threshold $\eta_{dis}$. 
With all the $n$ workers and $m$ landmarks in our system, a $n*m$ matrix $M$ with $m_{ij}= f_{w_i}^{l_j}$ is built, where $f_{w_i}^{l_j}$ is worker $w_i$'s familiarity score of landmark $l_j$.
Since the number of landmarks a worker has answered is always small compared with the large number of landmarks in the space, $M$ is very sparse.
Hence, if task assigning is only based on the sparse $M$, the assigning process has a strong bias to assign tasks to only a few well-performed workers.
Actually, workers who have similar profile information or have answered several similar questions are highly possible to share the similar knowledge. For example, if a worker $w_1$ has high familiarity score with $l_1, l_2$ and $ l_3$ and another worker $w_2$ living nearby  has high familiarity score with $l_1$ and $l_2$, $w_2$ is also likely to be familiar with $l_3$ though $w_2$ has not answered any question relating to $l_3$.
Therefore, we need to predict familiarity scores of workers on landmarks using the latent similarity between workers.
%Next paragraph we will introduce our algorithm to fill in more familiarity score into $M$ and make $M$ more densely.


The familiarity scores of different landmarks of workers are determined by some unweighed or even unobserved factors, which are regarded as some hidden knowledge categories, e.g. certain type of landmarks. However, we do not manually specify these factors, as hard-coded factors are usually limited and biased.
Instead, we assume the familiarity score of each worker-landmark pair is a linear combination of
two groups of scores, i.e. (1) how a worker is familiar with each hidden knowledge category, and (2) how a landmark
is related to each hidden knowledge category. Then we
employ Probabilistic Matrix Factorization (PMF)~\cite{mnih2007probabilistic} to factorize $M$ into two latent feature matrices, $W \in R^{d \times n}$ and $L^{d\times m}$, which are the latent worker and landmark feature matrices, respectively. 
That is,  $M = W^T L$,
where $W_{i,k}$ describes how familiar worker $w_i$ is with knowledge category $k$,
and $L_{j,l}$ describes how related landmark $l_j$ is to knowledge category $k$.
Further, we assume there exists observation uncertainty $R$, and the uncertain follows a normal distribution.
Thus the distribution of a new worker-landmark familiarity matrix $M'$, which predicts some familiarity by leveraging the similarity between different workers and landmarks, conditioned on $W$ and $L$ is defined as follows:

{\footnotesize
\begin{equation}
\label{equation:pmf1}
p(M'|W,L,{\sigma ^2}) = \prod\limits_{i = 1}^n {\prod\limits_{j = 1}^m {{{[\mathcal{N}({M_{ij}}|W_i^T{L_j},{\sigma ^2})]}^{{I_{ij}}}}} }
\end{equation}
}

where $\mathcal{N}(x|\mu, \theta^2)$ is the probability density function of the normal distribution with mean $\mu$ and variance $\theta^2$, and $I_{ij}$ is a indicator which is equal to 1 if $M_{ij}$ is not zero, otherwise 0.
The prior of $W$ and $L$ are defined as follows:
%Since Eq.~\ref{equation:pmf1} makes the use of non-zero values of $M$, in order to make the best use of $M$, the distribution of zero value on worker and landmark feature vectors are defined as following:

{
\begin{align*}
&p(W|\sigma_W^2)=\prod\limits_{i=1}^n \mathcal{N}(W_i|0,\sigma_W^2\boldmath{I} )\\ &p(L|\sigma_L^2)=\prod\limits_{i=1}^m \mathcal{N}(L_i|0,\sigma_L^2\boldmath{I} )
\end{align*}
}

where $\boldmath{I}$ is identity matrix.
The following objective function maximizes the posterior of $W$ and $L$ with regularization terms,
which minimizes the prediction difference between our model and the observed
$M$, and also automatically detects the appropriate number of factors $d$ through the regularization terms:

{\footnotesize
\begin{equation*}
\sum\limits_{i = 1}^n {\sum\limits_{j = 1}^m {{I_{ij}}{{({M_{ij}} - W_i^T{L_j})}^2} + } } {\lambda _W}\sum\limits_{i = 1}^n {\left\| {{W_i}} \right\|_F^2 + } {\lambda _L}\sum\limits_{j = 1}^m {\left\| {{L_j}} \right\|_F^2}
\end{equation*}
}

where $\lambda_W=\theta^2 / \theta_W^2$, $\lambda_L=\theta^2 / \theta_L^2$, and $\left\| {\cdot} \right\|^2_F$ denotes the Frobenius norm.
A local minimum of the objective function can be found by performing gradient descent in $W$ and $L$.
Afterwards, more familiarity scores between workers and landmarks are inferred in $M$.
%Using the decomposed matrices $W$ and $V$, we can predict a new worker-landmark familiarity matrix $R'$
%where $W$ is the worker latent feature $n*f$ matrix while $L$ is the landmark latent feature $f*m$ matrix.
%$f$, evaluated by RMF, is the number of latent features which affect the familiarity scores between workers and landmarks.


A worker with a familiarity score of a landmark means he has some knowledge about the region around the landmark, not just the  landmark itself.
As a result, the accumulated familiarity score $F_{w_i}^{l_j}$ of $l_j$ of a worker $w_i$ is a weighted sum of all the landmarks in the $\eta_{dis}$ range of $l_j$.
We assume the weight around a landmark $l$ follows a normal distribution of the distance to $l$,
and the region that the knowledge of $l$ can cover is limited in a circle with the center of $l$ and the radius of $\eta_{dis} $.
Thus, $F_{w_i}^{l_j}$ is evaluated as follows:

{\footnotesize
\begin{equation*}
F_{w_i}^{l_j} = \sum\limits_{l \in \mathbb{L}_{near}  \cup \{l_j\}} {\delta_{l}{f_{w_i}^l}}
\end{equation*}
}

where $\mathbb{L}_{near}$ is the set of landmarks in the $\eta_{dis}$ range of $l$.
The weight $\delta_{l} = \mathcal{N}(d(l,l_j)|0, \sigma^2_0)$
where $\sigma_0 = \eta_{dis}/3$.
We use $M^*$ to denote the worker-landmark matrix of the accumulated familiarity score, where $m^*_{ij}$ equals to $ F_{w_i}^{l_j}$.



%
%In order to formally
%However, the knowledge of a certain region of a person is hard to measure, so we defined familiarity score $f(l)$ of landmark
%It is a common sense that a native people always
%A place is familiar to a worker

%
%http://en.wikipedia.org/wiki/Voting_method
%Rated voting methods
%http://en.wikipedia.org/wiki/Cardinal_voting_systems

\subsection{Finding Top-k Eligible Workers}

Next we discuss how to find the top-k eligible workers for a given task.
%Each task is formed of a bunch of binary questions, that the system need to assign $k$ (system defines) workers the task.
Given a task (the selected $n$ landmarks $\mathbb{L}$), the worker-landmark accumulated familiarity score matrix $M^*$, a response time $t$, a positive integer $k$, a top-$k$ eligible workers query returns $k$ workers who have the most knowledge of landmarks in $\mathbb {L}$ among all the workers and have high possibility to finish the task within time $t$.


For a single landmark $l_j$, there may be several workers, denoted as $\mathbb{W}_{l_j}$, who have non-zero accumulated familiar scores, which means these workers have some knowledge of $l_j$.
For a task (a set of landmarks $\mathbb{L}$), $\bigcup \limits_{l\in \mathbb{L}}{\mathbb{W}_l}$ represents workers who have knowledge of any landmark of $\mathbb{L}$. 
Then we filter out workers, of who the possibility of finishing the task within time $t$ is no more than $\eta_{t}$, from $\bigcup \limits_{l\in \mathbb{L}}{\mathbb{W}_l}$. 
Afterwards the remained workers in $\bigcup \limits_{l\in \mathbb{L}}{\mathbb{W}_l}$ are regarded as candidate workers denoted by $\mathbb{W}$.
However, simply adding up a worker's accumulated familiarity scores on all the landmarks of $\mathbb{L}$ may lead biased result in worker selection.
For example, there are ten landmarks in a task and two candidates workers $w_1$ and $w_2$, that $w_1$ only has a very good knowledge of landmark $l_1$ , $F_{w_1}^{l_1}$=2) and knows nothing about the rest landmarks, $F_{w_1}^{l_i}=0$ ($2 \le i\le 10$), while $w_2$ has some knowledge of all the landmarks that $F_{w_2}(l_i)=0.1 $ ($1 \le i\le 10$).
Comparing the adding up sum of accumulated familiarity scores of the ten landmarks, $w_1$ will be selected to be assigned the task.
However, the coverage of $w_1$'s knowledge of the landmark set is too narrow, that $w_1$ may feel hard to answer questions about $l_2, l_3, \cdots, l_{10}$, in the knowledge coverage manner, $w_2$ is a better choice.
Thus, when selecting workers from candidate workers, not only their sum of accumulated familiarity scores of all the landmarks, but also the knowledge coverage of all the landmarks should be considered.
The choosing rules are quite similar to rated voting system~\cite{Doe:2009:Votingsystem}, of which the wining option is chosen according to the voters preferences score of options and the number of voters preferring the options. % and both the preference
In our system, we can treat each landmark of $\mathbb{L}$ as a voter and each worker of $\mathbb{W}$ as an option.
Adopting the idea of rated voting system, we can measure the landmark $l_j$'s preference of all the candidate workers as the following two steps: 1) rank workers of $\mathbb{W}_{l_j} \cap \mathbb{W}$, who  are in the candidate workers set $\mathbb{W}$ and have accumulated familiar scores $F_w^{l_j}$ bigger than zero, in descending order of $F_w^{l_j}$; 2) the preference score $p_{l_j}(w)$ of  $l_j$ to each worker $w$ in $\mathbb{W}_{l_j} \cap \mathbb{W}$ is defined as follows:

{\footnotesize
\begin{equation*}
p_{l_j}(w) = \left\{ \begin{array}{l}
 1 - \frac{{rank(w) - 1}}{{|W_{l_j}|}},if~w\in W_{l_j} \\
 0,otherwise \\
 \end{array} \right.
\end{equation*}
}

where $rank(w)$ is the ranked place of $w$ among $\mathbb{W}_{l_j} \cap \mathbb{W}$.
In this way the worker with high accumulate familiarity score will get a relatively high preference score and ensure the preference score will not result in a bias in worker selecting.
Afterwards, all the landmarks will vote their preferences to the candidate workers, at this time we sum up the preferences of each worker voted by landmarks and then the workers with the top-$k$ biggest adding up preference scores will be the query results.



==> 1 IEEE_Paper_LaTeX_Template_LETTER_V2 20130719/introduction.tex <==

\section{Introduction}

Travelling plays a vital role in our daily life. 
Thanks to  the rapid development of GPS technologies and flourish of navigation service providers (e.g., Google Map, Bing Map, TomTom), we can now travel to unfamiliar places with much less effort, by simply following the recommended routes. While the detailed mechanisms that are adopted to recommend routes are different, travelling distance and time are the most important criteria and factors in those recommendation algorithms, which results in the shortest route and/or fastest route. With increasing number of users who rely on these map services to travel, a natural question arises: {\em are these routes always good enough to be the best choice when people travel?} Ceikute et al~\cite{Ceikut2013Routing} are the first to assess the routing service quality by comparing the popular routes, the ones most drivers prefer, and the  routes recommended by a big thumb map service provider. Their results show that the there are big distances between popular routes and recommended routes. It concludes that experienced/frequent drivers' preferences do not always agree with the routes recommended by navigation service. Actually the cause of this phenomenon is not difficult to find out: drivers preferences are influenced by lots of factors in addition to distance and time, such as the number of traffic lights, speed limitation, road condition, weather, amongst many others, which are very difficult to be taken into consideration simultaneously by a single routing algorithm. That is to say, driver's preference is the ultimate criterion to judge the goodness of a route, i.e., given a source and a destination, route $A$ is regarded as a better choice than route $B$ if more drivers prefer to drive along  $A$ for some reasons. 

{\em Then can we find the most popular routes between two places and return them to the users?} Ideally the routes recommended in this way should have improved quality since the popular routes are usually obtained by mining historical trajectories of drivers and can better  indicate the driver's preference. But after further investigation, we have observed some problems of this approach. First, since users can specify two arbitrary places as source and destination, it happens that we cannot get enough support from historical trajectory data to obtain reliable results. Even worse, in areas where historical data are very sparse, the ``popular'' route can refer to a bad one with some random historical data. Therefore, a system that solely relies on those popular routes can perform badly at large scale. Second, there exist a number of popular route mining algorithms, each claiming some superiority from certain perspectives. When the results of these algorithms disagree with each other, it is still a pain for strangers to make a wise choice.
%This might be due to an increase in the possible routes between sources and
%destinations that are further apart. 
%Leichen's popular route mining algorithm has the smallest similarity against the recommended routes. 
%The root cause of this phenomenon is that Leichen's algorithm is sensitive to querying time. 

%
%\begin{figure}[h]
%\centering
%\includegraphics[width=7cm]{fig/introduction2.eps}
%\caption{Similarity between routes obtained from map services and popular route mining algorithms}\label{fig:introduction2}
%%\subfigure[Precision without selecting worker ]{
%%\includegraphics[width=4cm]{fig/precisionwithoutselectingworker.eps}\label{fig:precisionwithoutselectingworker}
%%}
%%	\caption{Precision of route evaluating }
%	%\label{fig:answerquestion}
%\end{figure}


As we can see from the above analysis, it is not uncommon that routes recommended by different ways disagree with each other. This makes choosing the best route to be a very subjective question, which is hard for a computer algorithm to answer. Inspired by the emerging concept of crowd sourcing that explicitly leverages human knowledge to resolve complex problems, we propose a novel crowd-based route recommendation system -- CrowdPlanner, which combines the strengths from computers and human brains to recommend the best route with respect to the knowledge of experienced drivers. Instead of proposing new or optimizing existing routing algorithms, our work takes an entirely different approach by consolidating candidate routes from different sources (e.g., map service providers, popular routes) and requesting experienced drivers to select amongst them. Our system will return the most promising one according to the selection of drivers. 

%the route recommendation services powered by mainstream searching engines and GPS modules in our cars, we can travel to unknown places by simply typing in our start place and destination and then following their guidance. 
%A pleasant trip desires them to provide good route, since our trip entirely replies on them. 
%
%How to tell a recommended route is good? 
%There are no uniform rules to tell what a good recommended route is like, since there are too many latent factors, such as the number of turns, traffic lights, speed bump and so on, affecting the quality of a recommended route. 
%Obviously, without clear rules, computers fail in judging the quality of the recommended routes.
%So the best and the only way to judge the quality of the recommended routes are the drivers' preference, i.e., if more drivers prefer to drive along route $A$ than route $B$ between two certain places because of many unknown factors, we regard $A$ has a better quality than $B$. 
%Therefore, many research efforts~\cite{lee2007trajectory,jeung2008discovery,jeung2008convoy,li2010swarm} have been taken in mining popular routes or frequent moving patterns from a large amount historical trajectories, which are the motion history of moving objects collected by sensors such as GPS-enabled mobile and wireless communication. 
%Let us see how likely it is between users' preferences (popular routes between two certain places) and routes recommended by web services and GPS modules. 
%According to~\cite{Ceikut2013Routing}, which employs ? popular route detection method in the city of North Jutland, Denmark, the similarities between the routes recommended by a big thumb map company and the routes drivers prefer decrease with the growth of the trip length, that the similarities are below 50\% when the lengths of the trips beyonds 20 kilometers. 
%It gives the evidence that the routes recommended by web services and GPS modules are not always reflect the local drivers' preferences, which means they not always provide the best routes. 

%Base on the report, some people may think `it is easy to recommend the best route, just recommend them the popular route you mined '. 
%However, we can not straightforwardly do so because of the following two reasons: 
%1) due to the uneven distribution of historical trajectories, not all the mined popular routes are that `popular' (not frequent enough), that overreliance on mined popular routes may lead bias in route recommendation; %using a certain mining algorithm;
%2) we have mentioned that many algorithms have been proposed in popular routes mining, that they always recommend different popular routes between two places and claimed that their own algorithms are the best from several different perspectives, i.e., their mined popular routes changing in different hours of a day or applying trajectory segmentation methods before clustering.
%Since the mined popular routes always can not agree to each other, their mined different popular routes together with the routes recommended by web services form the candidates set of the best route. 
%
%{\bf our paper rank the candidates by using the knowledge stored in computers, while cannot judge will ask other experienced people to rank the route}

%\subsection{Problem Analysis: A Case Study}
%Now let us examine the difference between the route recommended by web services and the popular routes mining algorithms. 


%The disagreements among popular routes mining algorithms are shown in Figure~?.
%Also, with the increasing of the length of the routes, these mined popular routes become more different. 
%And Leichen's method is always different from any other two methods. 
%
%In conclusion, the recommended routes provided by web services are quite different from people's real preferences. 
%And the current popular routes recommendation methods always detect different human preferences.

%\subsection{Challenges and Contributions}
%With the observation and awareness of the difference between recommended routes of web services and human preferences, and the differences results provided by different human preference detection algorithms, a {\em route evaluating} process is necessary, which rates the confidence level of a route to be best, for the purpose of giving users the best routes.
%In order to achieve this goal, we need to publish a survey, gather the surveyors' route preferences and return the statistical result. 



It is a non-trivial task to perform route evaluation. 
First, it is not easy to automatically publish a user friendly task.  
Since the human's knowledge of routes are quite different from computers, that is human remember routes discretely while computer process routes continuously. 
So the system should intelligently select some typical points of the comparing routes instead of giving the continuous routes for surveyors to choose from.
Second, we should select the workers to ensure the quality of the task result since the quality of route evaluation is largely relying on the traveling experience of the workers. 

 
In this paper, we propose a {\em CrowdPlanner system} for recommending the evaluated best route.
It comprises two layers: a mobile client supporting users to send a route recommendation request and answering surveys; 
a server which possesses the request by generating recommendation route candidates, evaluating candidate routes itself using existing evaluated routes and publish a route recommendation task. 
Especially in publishing a route recommendation task, a efficient question selecting and ordering method is proposed, which selects a set of significant landmarks to help workers select the their most recommend route;
an effective worker selecting method is also proposed in order to assign each task to its most familiar and eligible workers. 

To sum up, we make the following major contributions. 
\begin{itemize}
\item We make a key observation that the cognition of routes of humans is quite different from computers, that humans recognize routes by concrete points while computers recognize routes by continuous lines. 
\item We recommend the verified best route between two places to users, while the routes recommended by route recommendation web services are different from humans' preference and the different popular route detection algorithms provide different popular routes. 
\item We conduct extensive experiments based on hundreds of volunteers and  large-scale real
trajectory dataset, which empirically demonstrates that the
CrowdPlanner system can always provide best route between places efficiently and the survey mechanism is intelligent and user friendly. 
\end{itemize}









==> 1 IEEE_Paper_LaTeX_Template_LETTER_V2 20130719/landmarkselecting.tex <==
\section{Task Generation} \label{sec:generatequestion}
%The question generating of CrowdPlanner is quite different from traditional Crowdsourcing systems, since we can not require



Almost everyone has the experience that you can not explain a route clearly to someone, even you know exactly how to get there in mind, %may still confuse even though the passengers gives the right information when you ask them for the ways.
which implies  describing a route concretely is hard for human. %A major reason of it is that it is hard for the workers to describe a route.
%Taken the query travel from $p_a$ to $p_b$ shown in Fig ? as example, workers have various descriptions of their prefer route, i.e., ?, ? and ?.
Therefore we can not simply publish a task to workers that requires them to describe the best route in a turn-by-turn manner. % of travel from one place to another.
As an alternative and more friendly way, we may provide several pictures, which demonstrate these candidate routes on a map, as multiple choices for workers to choose.
Taken the route recommendation request in Fig.~\ref{fig:routes} as example, we publish a multiple choice question to workers by showing four routes on a map and ask them to pick the route they most prefer. 
%Taken the route recommendation request in Fig.~\ref{fig:routes} as example, we publish a multiple choice question to workers by showing routes $R_1=[l_1,l_2,l_4,l_8,l_9]$, $R_2=[l_1,l_2,l_5,l_6,l_8,l_9]$ , $P_3=[l_1,l_3,l_6,l_8,l_9]$ and $R_4=[l_1,l_3,l_7,l_9]$ on map and ask them to pick 
Although all the routes have been visualized on a map, it still requires lots of efforts to realize the differences among all candidate routes, especially when they use smartphones with small screens to do this job. 
%An easy  should summarize the significance differences among candidate routes instead of taking workers' effort to find them.
%In order to reduce worker's effort in comparing the candidates routes, we should
%Following "the easier the better" rule to generate easy questions for workers.
%What kind of information on the routes should we summarize?
%We aware that a computer and a person will describe how to go to a place in totally different ways when you ask them for the way, that the computers describe a route using the continuous pattern {\em road + road}, 
%while humans describe a route using the pattern {\em landmark + landmark}. 
We observe that  humans like to use a set of significant locations, i.e., landmarks, to describe a route in high level rather than a sequence of continuous roads as computers do. So to make the question easier to answer, we  summarize the candidate routes using landmarks and present the differences to workers, instead of asking them to find out by themselves. 
%In order to attune to people's way of thinking, we need to summarize several significant landmarks, that people can simply describe the landmarks to uniquely identify their most recommended route.
Besides, how the questions are presented can also affect the complexity of a task. 
%Summarizing landmarks reduces the difficulty of the content of a task, however, the question format also affects the difficulty of a task a lot. 
For example, a multiple choice question with all candidate routes is more difficult to answer than a couple of binary questions such as `` do you prefer the route passing landmark $A$ at 2:00pm?'', since~\cite{su2012crowdsourcing} pointed out that several binary choice questions are easier and more accurate than a multiple choice question. % so the generate question component tries to generate binary choice questions, i.e., do you need to pass by Huangzhuang Station when you travel from Sigma Building to Peking University, otherwise the component will generate multiple choice questions.
%What's more, a multiple choice question results in higher error rate or sometimes 
%An easy task of Fig ? can be two binary choice questions, that the first one is "do you need to pass by $landmark_a$ high way when you travel from $p_a$ to $p_b$?" and the second one is "do you need to pass by $landmark_b$ suburb when you travel from $p_a$ to $p_b$", where $landmark_a$ and $landmark_b$ are two well known landmarks.
Based on the above analysis, we will generate a task as a sequence of binary question, each relating to a landmark that can discriminate some of the candidate routes. 

\begin{figure}[h]
\centering
	{\psfig{figure=fig/routes.pdf,width=75mm} }
	\caption{An example of landmark-based recommended routes between $l_1$ and $l_{10}$}
	\label{fig:routes}
\end{figure}


In this section, we will present in detail our task generation process, which can be divided into three phases: inferring landmark significance, landmark  selection and question ordering.
Specifically, the first phase infers the significance for each landmark which indicates people's familiarity with it. %coefficient.
%The trajectory rewriting phase rewrite route using the landmarks it passes by.
The second phase tries to use a set of most significant landmarks to summarize the difference among the candidate routes.
The third phase generates the final task by ordering the questions in a smart way so that the expected number of issued questions is as small as possible. 

\subsection{Inferring Landmark Significance}

It is a common sense that landmarks has different significances. For instance, the White House is world famous, but Pennsylvania Ave, where the White House is located on, is only known by some locals of Washington DC.
People tend to be more familiar with the landmarks that are frequently referred to by different sources, e.g., public praise, news, bus stop, yellow pages. In this work, we utilize the online check-in record in a popular location-based social network (LBSN) and trajectories of taxicabs in the target city to infer the significance of landmarks, since these two datasets are large scale enough to cover most areas of a city. By regarding the travellers as authorities, landmarks as hubs, and check-ins/visits as hyperlinks, we can leverage a HITS-like algorithm such as~\cite{zheng2009mining} to infer the significance of a landmark. Readers who are interested in the technical details can refer to~\cite{zheng2009mining}. 
%We can adopt the algorithm in~\cite{zheng2009mining}, which inferences the interesting locations by involving the concepts of HITS, to derive the significance of landmarks, denoted as $l.s $, where $l$ is a landmark.
%In our model, a hub can be either a check-in service user or a transportation driver and an authority is a
%location which has been check-ined/visited by many people. %, which can be generated by clustering check-in data and stop points mining from historical trajectory.
%Notably, as we need to compare the significances of all the landmarks equally regardless their relative significances of their regions, which is considered in ?, we use the plain interest values, lowest level location interest values, as the significances of landmarks.


%\subsection{ Rewriting Route}
%The current candidate routes are represented by discrete road intersections, just like Figure ? shows, that route $A$ is represented by $[t_1, t_2, t_4]$.
%In order to select the most significant landmark set $S$, we first need to find out which landmarks each route passes, which in other words is rewriting routes using landmarks.
%After rewriting using landmarks, route $A$ should be represented by $[l_1, l_2, l_3]$.
%%The route rewriting should keep the shape of the original route and connect all the passing by landmarks.
%We can adopt the Model-based Calibration method of ?, which rewrite sample-based trajectories into anchor-based trajectories, to rewrite the road-intersection-based routes into landmark-based routes, that the method can keep the shape of the original route and connect all the passing by landmarks.




\subsection{Landmark Selection}




%%??????????
%We have introduced that binary question is best question type of Crowdsourcing tasks due to its easiness and low error rate.
%According to this rule, our system will ask a series of binary questions, i.e., ``whether you need to pass landmark $l_1$ when you go from $p_1$ to $p_2$'' of Figure ?, to get workers' traveling preference.
%We will ask several binary questions
%We have introduced why we need to summarize the differences between candidate routes using landmarks and use these landmarks as question.
Although any landmark can be used to generate a question, not all of them are suitable for the purpose of generating easy questions given a certain candidate route set $\bar{\mathbb{R}}$ (notably in this section we rewrite all the routes in $\mathbb{R}$ into landmark-based routes so we use $\bar{\mathbb{R}}$ to denote the candidate route set).
First, the selected landmark set $\mathbb{L}$ should be discriminative to the candidate routes $\bar {\mathbb{R}}$, which ensures that the difference between any two routes can be presented. % that is for each landmark-based candidate route $\overline r$, the join set $\overline r \cap \Omega $ should be different from any other candidate routes.
%For example, $\Omega =[l_3, l_4]$ can uniquely identify $\overline {r_1}=[l_1, l_2, l_3]$ and $\overline {r_2}=[l_1, l_2, l_4]$, since the join sets of $ \overline {r_1}$ is $[l_3]$ and the join set of $\overline {r_2}$ is $[l_4]$, while $\Omega =[l_1, l_2]$ can not.  {\bf HOW TO EXPLAIN}
Second, the landmarks of $\mathbb{L}$ should have high significance, so that more  people can answer the question accurately. % judge whether they should pass it on a specific travel and more reliable the answers are.
Third, in order to reduce the work load of workers, the selected landmark set $\mathbb{L}$ should be as small as possible.
Therefore the problem of landmark selection is to find a small set of highly significant landmarks which are discriminative to all the candidate routes.
It can be formally represented as an optimization problem in below. \\
{\bf Given} $n$ landmark-based candidate routes $\bar {\mathbb{R}}$, and the significance of each landmark\\
{\bf Select} a landmark set $\mathbb{L}$ with the size of $k$ ($\left \lceil \log_2 (n)\right \rceil \le k \le n$) which is discriminative to $\bar{\mathbb{R}}$
\\
{\bf Maximize} $\sum\nolimits_{l \in \mathbb{L}} {l.s}\cdot |\mathbb{L}|^{-1}$\\
Here, the target function aims to maximize the product of two opposite factors: $\sum\nolimits_{l \in \mathbb{L}} {l.s}$, which is proportional to the sum of significances of $\mathbb{L}$ and $ |\mathbb{L}|^{-1}$, which is inversely proportional to the size of $\mathbb{L}$.
% indicate where  $e^{-k}$ indicates the less landmarks the better and  $\sum\nolimits_{l \in \Omega} {l.s}$ is to choose the most significant sets.
%$k$ ranges from $\left \lceil \log_2 (n)\right \rceil $ to $n$.
%Since $\mathbb{L}$ with size of $k$ has $2^k$ subsets and the join set $\bar R\cap \mathbb{L}$ is a subset of $\mathbb{L}$, $2^k$ must be no less than $n$ in order to avoid any two routes of $\bar{\mathbb{R}}$ have the same join set.
%It is possible that $k > n$, but in order to reduce the number of questions we set $k \le n$, since there definitely exists a landmark set $\mathbb{L}'$ satisfying  $|\mathbb{L}'|  \le n$ which is discriminative to $\bar{\mathbb{R}}$.








Due to the trade-offs between maximizing accumulate significance of the selected landmark set $\mathbb{L}$ and minimizing the size of $\mathbb{L}$ as well as  the restriction that $\mathbb{L}$ must be discriminative to $\bar{\mathbb{R}}$,  it is non-trivial to generate $\mathbb{L}$.
%There is no easy way to calculate the best landmark set.
A straightforward method is to enumerate all the landmark combinations of $\bigcup\limits_{\bar R\in \bar{\mathbb{R}}}{\bar R}$ and find a discriminative landmark set with the maximized target value. % calculate the best landmark set $S$ is to find out all the possible landmark set $\overline{S}$, that $\overline{S}$ can uniquely identify the candidate $n$ routes and $|\overline{S}| \le n$, calculate the target value of $\overline{S}$ and return the set with maximum target value.
However, the time cost grows exponentially with the size of landmark set, rendering this method impractical. 
To speed up this process,  we propose two landmark selecting algorithms, called Incremental Landmark Selecting and GreedySelect.  
%a natural idea is to not visit all the landmark combinations and quickly find a tight upper bound of a bunch of non-accessed combinations since there is only one set which is finally selected.
%%A natural idea is to quickly find a tight upper bound of a bunch of sets to determine whether the rest of the sets need be computed or not.
%So our propose a landmark selecting method GreedySelect.
%Before we detailed the GreedySelect, we first introduce the following lemma:
%\begin{lemma}\label{lemma:discriminative}
%%If a landmark set $\Omega$ cannot uniquely identify candidate routes, nor its subset $\Omega_{sub}$ can, which is equivalent to that
%If a subset $\mathbb{L}_{sub}$ of $\mathbb{L}$ is discriminative to $\bar{\mathbb{R}}$, so as $\mathbb{L}$.
%\end{lemma}
%\begin{proof}
%%There exists a subset $\Omega_{sub}$ of $\Omega$, where $\Omega$ cannot uniquely identify candidate routes set $\Re $ while $\Omega_{sub} $ can.
%According to the definition of discriminative, all the join sets $\bar R\cap \mathbb{L}_{sub} $, $\bar R\in \bar{\mathbb{R}}$, should be different.
%The join set $\bar R \cap \mathbb{L}$ can be calculated as the union of two part $\bar R \cap \mathbb{L}_{sub}$ and $\bar R \cap (\mathbb{L} -\mathbb{L}_{sub})$.
%Since the first parts of all the join sets $\bar R \cap \mathbb{L}$ are different, $\mathbb{L}$ can uniquely identify the candidate routes.
%%Thus all the join sets $r \cap \Omega$ are different since
%\end{proof}


\subsubsection{Incremental Landmark Selecting}

The main idea of ILS is to select several {\em simplest discriminative landmark} sets, each of which has different size (from $\left \lceil \log_2 n \right \rceil$ to $n$). 
The selected simplest discriminative set  of size $k$ % that each set $\overline c$ 
has the maximum objective equation value among all the simplest discriminative landmark sets of size $k$. %sets of size $|\overline c|$ and obtain the best landmark set basing on the  n-$\left \lceil \log_2 n \right \rceil$+1 sets.
And then ILS can obtain the best landmark set using the selected simplest discriminative landmark sets.

At the very beginning, we need to roughly filter out some non-benificial landmarks which are on/ not on every candidate route. 
The beneficial landmarks set of $\bar {\mathbb{R}}$ can be generated as following:
$\mathbb{L} = \bigcup\limits_{\bar R \in \bar {\mathbb{R}}} {\bar R}  - \bigcap\limits_{\bar R \in \bar {\mathbb{R}}} { \bar R} $.
Because of optimization requirements, we sort $\mathbb{L}$ in descending order of their significances.
Notably, the sorted landmarks should be not stored in a set, but for convenience we still use $\mathbb{L}$ to denote to sorted beneficial landmarks.
We denote the selected simplest discriminative set of size $k$ by $\mathbb{L}_{sim[k]}$. % denote the combinations of landmarks with size of $k$ and the landmark combination with the maximum target value among all the discriminative combinations of $C_{k}$ respectively (line 3-4).
The aim of the step is to find best landmark set $\mathbb{L}_{\bar {\mathbb{R}}}$ using $\mathbb{L}_{sim[k]}$, where $k$ ranges from $\left \lceil \log_2 n \right \rceil$ to $n$.
The discriminative set $\mathbb{L}_k$ of length of $k$ with maximum objective equation value can be calculated using $\mathbb{L}_{sim[i]}$ ($\left \lceil \log_2 n \right \rceil \le i \le k $) as following:
\begin{equation*}
\mathbb{L}_k = \arg \mathop {\max }\limits_{\left \lceil \log_2 n \right \rceil \le i \le k}{GetValue(GetMaxSet({\mathbb{L}}, k, \mathbb{L}_{sim[i]}))}
\end{equation*}
%where $\overline{\mathbb{L}}$ is the sorted benificial landmarks,  that a non-benificial landmark is on/ not on every candidate route since a question asking a worker whether he would pass the landmark does not provides any information for us to determine which candidate route is best, in descending order of their significances (line 1-2).
%The beneficial landmarks set of candidate routes set $ \Re$ can be generated as following:
%$\nabla = \bigcup\limits_{r \in \Re} {r}  - \bigcap\limits_{r \in \Re} { r} $.
where the $GetMaxSet({\mathbb{L}}, k, \mathbb{L}_{sim[i]})$ is a function which returns the superset of $\mathbb{L}_{sim[i]}$ with the maximum objective equation value among all the $\mathbb{L}_{sim[i]}$'s supersets of size $k$ and 
$GetValue(\cdot)$ is a function which returns the objective equation value of $\cdot$.
$\mathbb{L}_k$ must be discriminative to $\bar {\mathbb{R}}$. %so the calculation of $Best[i]_k$ is quite easy, illustrated in Algorithm~?, since $\Im$ is sorted.
Since the $\mathbb{L}$ is sorted, $GetMaxSet({\mathbb{L}}, k, \mathbb{L}_{sim[i]})$ has the time complexity of $O(1)$. 
%GetTargetValue($c$) is a function which returns the target value of $c$.
Afterward, $\mathbb{L}_{\mathbb{R}}$ can be  generated as following:
\begin{equation*}
\mathbb{L}_{\mathbb{R}} = \arg \mathop {\max }\limits_{\left \lceil \log_2 n \right \rceil \le k \le n}{GetValue(\mathbb{L}_k)}
\end{equation*}
In the sequel, we will discuss how to obtain $\mathbb{L}_{sim[i]}$.


In order to obtain all the $\mathbb{L}_{sim[i]}$, we use a ``bottom up" approach, of which landmark sets are extended from size one to size $n$ by adding one landmark at a time and groups of landmark sets are tested.
%The algorithm starts at the landmark combinations of the smallest size, $\left\lceil \log_2 n \right\rceil$ ,  and terminates when the size of the landmark combinations is $n$.
Let $\mathbb{S}_{k}$ denote a set forming by several landmark combinations with the size of $k$.
The $\mathbb{L}_{sim[k]}$ generating can mainly divided into three steps.
(1) Start step: the algorithm start from $k= 1$, thus $\mathbb{S}_{1}$ stores all the combinations of each single landmark  of size $1$.
(2) Calculating step: then the algorithm tests whether each combination $S \in \mathbb{S}_{k}$ is discriminative.
Among all the discriminative sets of $\mathbb{S}_k$, the set with the maximum objective equation value assigns to $\mathbb{L}_{sim[k]}$.
Afterward all the discriminative combinations of $\mathbb{S}_{k}$ and their superset are pruned and removed from $\mathbb{S}_{k}$, since their superset are all discriminative  and their maximum objective equation value can be easily generated from $\mathbb{L}_{sim[k]}$. %,due to lemma~\ref{lemma:discriminative}
%, if so, it assign the maximum discriminative closure set of $C_{k}$ to $Best[k]$ is the maximum discriminative closure set of $C_{k}$.
(3) Expansion step: If $k$ equals to $n$, the algorithm stops.
Otherwise we generates $\mathbb{S}_{k+1}$ from $\mathbb{S}_{k}$, which consists of all the undiscriminative landmark sets of size $k$.
Adding a new landmark $l$ ($l \in \mathbb{L}-S$) to $S$ ($S \in \mathbb{S}_k$) will form a element $S'$ of $\mathbb{S}_{k+1}$. 
However, the expansion cause same sets being generated several times, i.e., $\{l_1\}$ expends $l_2$ to $\{l_1, l_2\}$ and $\{l_2\}$ expends $l_1$ to $\{l_1, l_2\}$ too.
So we restrict the significance of adding landmark $l$ must be less than the significance of any landmark of $S$.
%A new set $S_j \in \mathbb{S}_{k+1}$ is generated by adding a new landmark $l$ not in $S_i$ using following equation
Thus $\mathbb{S}_{k+1}$ can be generated as following:
\begin{equation*}
\mathbb{S}_{k+1}=\{S'|S'=S \cup \{l\} \wedge l.s \le \min\limits_{l'\in S}{l'.s} \wedge l\in \mathbb{L} -S \wedge S\in \mathbb{S}_k\}
\end{equation*}
and repeat step 2.
 %   landmark combinations of $C_k$.



\subsubsection{GreedySelecting}

The main idea of GreedySelecting is to incrementally adding a landmark with the highest significance among the possible landmarks to an discriminative landmark set and use some tight upper bounds to prune many landmark sets with low significance values.    
%select several {\em simplest discriminative landmark} (Dif~\ref{define:Simplestdiscriminative}) sets, each of which has different size (from $\left \lceil \log_2 n \right \rceil$ to $n$). 
%The selected simplest discriminative set  of size $k$ % that each set $\overline c$ has the maximum objective equation value among all the simplest discriminative landmark sets of size $k$. %sets of size $|\overline c|$ and obtain the best landmark set basing on the  n-$\left \lceil \log_2 n \right \rceil$+1 sets.
%And then GreedySelect can obtain the best landmark set using the selected simplest discriminative landmark sets.
%The Algorithms~\ref{algo:Apriori} and \ref{algo:Nextdiscriminative} illustrate  the main structure of GreedySelect.
Let $S$ denote the current testing landmark set and
$\mathbb{L}_{best}$  the best landmark set which is discriminative and has the highest target value.
The landmark selection process can be divided into three steps:

{\bf Preparation step:} at the very beginning, we need to roughly filter out some non-beneficial landmarks, the ones cannot identify any routes of $\bar{\mathbb{R}}$. 
A straightforward way is to filter out landmarks which are on/ not on every candidate route. 
Thus the beneficial landmarks set of $\bar {\mathbb{R}}$ can be generated as following:
$\mathbb{L} = \bigcup\limits_{\bar R \in \bar {\mathbb{R}}} {\bar R}  - \bigcap\limits_{\bar R \in \bar {\mathbb{R}}} { \bar R} $.
Because of optimization requirements, we sort $\mathbb{L}$ in descending order of their significances.
Please note the sorted landmarks should be not stored in a set, but for convenience we still use $\mathbb{L}$ to denote to sorted beneficial landmarks.

{\bf Expansion step:} this step generates the test landmark set $S$. 
We recursively generate the test landmark set $S$, as shown in Algorithm~\ref{algo:expansion}.
In this step, we find all the landmarks not in $S$,
pick non-added biggest landmark of them, and add it to $S$.
Once the $S$ is discriminative, we stop adding landmark to it and roll back to previous level recursion.
Since the same $S$ may be generated in different order, to eliminate duplication, 
we only consider those landmarks with a lower significance than any element in $S$.
The process stops when all the possible combinations have been visited. 
\begin{algorithm}
\small
\caption{expansion}\label{algo:expansion}
\If{$|S|=n$}{
	stop or $S \gets $ landmark with the next biggest significance;
}
\Else{
	 $SetOfS \gets$ <- all the landmarks has a lower sinificance than any landmark of $S$;
	 
	 Sort $SetOfS$ in descending order of the significances of landmarks; 
	 
	 \For{each $l \in SetOfS$}{
	 	\If{$S \cup \{l\}$ is not discriminative}{
	 		expand($S\cup \{l\}$);
	 	}
	 }	 
}
\end{algorithm}


%If $|S|$ equals to $n$, then the $S$ will be assigned a landmark, which has not been only assigned to $S$, of $\mathbb{L}$, that if all the landmarks of $\mathbb{L}$ have been solely assigned to $S$, the algorithm stops;
%if $S$ is discriminative, then the previously added landmark $l_{pre}$ of $S$ will be removed and a new landmark $l$ ($l \notin S$) will be added to $S$;
%otherwise $S$ is generated by adding a landmark $l$ ($l \notin S$), to the previous $S$.
%However, the expansion cause same sets being generated several times, i.e., $\{l_1\}$ expends $l_2$ to $\{l_1, l_2\}$ and $\{l_2\}$ expends $l_1$ to $\{l_1, l_2\}$ too.
%So we restrict the significance of adding landmark $l$ must be less than the significance of any landmark of $S$.
%%A new set $S_j \in \mathbb{S}_{k+1}$ is generated by adding a new landmark $l$ not in $S_i$ using following equation
%Thus $\mathbb{S}_{k+1}$ can be generated as following:
%
%{\footnotesize
%\begin{equation*}
%{\rm{S}} = \left\{ \begin{array}{l}
% l,~if~|S| = n ~ \wedge~ \mbox{\em l has not been solely assigned}\\ 
% S -\{ l_{pre}\} \cup \{ l\}, if ~ |S|<n \wedge S~ is ~discriminative \\
% ~~~~~~~~\wedge l_{pre}~ is~ the~ previous~ added~ landmark~\\
% ~~~~~~~~ of~ S  \wedge l \notin S  \\
%  S \cup \{l\}, if~ |S|<n \wedge S~ is ~undiscriminative \wedge l \notin S \\
% \end{array} \right.
%\end{equation*}
%}

{\bf Test step:} this step tests whether $S$ is discriminative.
If $S$ is discriminative, calculate the maximum target value $m$ of $S$ and the supersets of $S$ and if $value$ is bigger than the current maximum target value $maxValue$, then the set with target value $value$ among $S$ and the super sets of $S$ will be assigned to $\mathbb{L}_{best}$.
Afterwards the supersets of $S$ do not to be visited since their are all discriminative and their maximum target value will be no more than $value$. 
Thus all the landmarks of $S$ will be removed, which in other words $S$ will be assigned as $\emptyset$. 





However, the above two algorithms can be very time consuming when the size of $\mathbb{L}$ and $n$ are large, since there will be a large amount of landmark sets to be tested.
In order to improve the efficiency, we need to filter out more non-beneficial landmarks in the preparation step, generate $S$ more intelligently by avoiding duplication in the expansion step and test less $S$ which prunes many insignificant enough landmark sets and their supersets in the test step.
%To generate less combinations, it is important to filter out some less significant landmarks at start step; 
%it is important to limit the expansion of landmark combinations of $\mathbb{S}_{k}$  by  adding  landmarks which make contribution to distinguish routes and avoiding adding landmarks which form supersets of discriminative sets already being pruned when generating $\mathbb{S}_{k+1}$ in expansion step. 
%To test less combinations, it is important to filter out some insignificant combinations by using some upper bounds. 
%To generate less combinations when we generate the $\mathbb{S}_{k+1}$ in expansion step, we need to limit the expansion of landmark combinations of $\mathbb{S}_{k}$  by  adding  landmarks which make contribution to distinguish routes and avoiding adding landmarks which form supersets of discriminative sets already being pruned. %of size of $\left\lceil \log_2 n \right\rceil, \left\lceil \log_2 n \right\rceil+1, \cdots , k-1 $.
%For example, ?.
Next we will present the optimizations for each step respectively for both algorithms. 
%We explain how to test less combinations and how to select landmarks to be added to each set at expansion step in the next two parts.


\subsection{Question Ordering}

In the previous step we select questions (landmarks), which can be regarded as the {\em question library}.
However, presenting those question to workers with random order is unwise
%Sorting the order of questions is important b
because of the following two reasons:
1) it is not necessary to ask all the questions in most cases. For example, in Fig~\ref{fig:routes} if a worker indicate he prefers the routes passing $l_2$ from $l_1$ to $l_{10}$,  we do not need to ask whether he recommend to pass $l_8$ since all the routes passing $l_2$ do not pass $l_8$;
2) each time we ask a question, we would like to obtain the most informative feedback, which is more likely to indicate the final answer. 
%Different questions result in different information gain, because the entropies of the candidate routes set of different questions are different and questions with different significances leads to different answer error rates since workers tend to have better knowledge of landmarks with higher significances.
This implies that 1) the next question to be asked depends on the result of the previous question, so the question order is a tree-like structure, denoted by $\mathcal{T}$;  %, of which decision tree ? is a perfect structure to model the question-answer flow.
%Each time we ask a question, we would like to get maximum workers\rq{} recommendation information which is known as information gain
%What is more important
 2) the information strength of a question $q$ is proportional to people's familiarity of a landmark (the significance of the landmark) and the power of filtering of a landmark (the information gain of the candidate routes set using the landmark).
%Given a question library $\mathcal{ Q}$ and a candidate routes set $\Re$, we treat each question as an attribute
% a decision node
%non-leaf node) and each candidate route as a label
% end node
%(leaf node) of the question decision tree $\mathcal{T}$.

The information strength $IS(l_{k_i})$ of question $l_{k_i}$ is defined as following: % $S(q)$ of question $q$ is defined as following:
{\footnotesize
\begin{align*}
IS(l_{k_i})= & l_{k_i}.s [H (\bar {\mathbb{R}}_{k-1}) - \textstyle{\bar {\mathbb{R}}_{k}^+ \over \bar {\mathbb{R}}_{k}^+ +\bar {\mathbb{R}}_{k}^-}H (\bar {\mathbb{R}}_{k}^+) -\textstyle{\bar {\mathbb{R}}_{k}^- \over \bar {\mathbb{R}}_{k}^+ +\bar {\mathbb{R}}_{k}^-}H (\bar {\mathbb{R}}_{k}^-) ]
\end{align*}}
%The information gain $IG(l)_{\Re_{prev}}$ both considering the entropy change from previous routes set $\Re_{p}=\Re_{q_{k_1}^{+/-}q_{k_2}^{+/-}\cdots q_{k_i}^{+/-}}$ to split two subsets $\Re_{+}=\Re_{q_{k_1}^{+/-}\cdots q_{k_i}^{+/-}q_{k_{i+1}}^{+}}$ and $\Re_{-}=\Re_{q_{k_1}^{+/-}\cdots q_{k_i}^{+/-}q_{k_{i+1}}^{-}}$ on a questioned landmark $l$ and the significance of $l$ is recursively defined as following:
%\begin{equation*}
%IG(l)_{\Re_{p}}= e^{l.s} \cdot \left[ H(\Re_{p})-(\frac{|\Re_{+}|}{|\Re_{p}|}\cdot H(\Re_{+}) + \frac{|\Re_{-}|}{|\Re_{p}|}\cdot H(\Re_{-}))\right]
%\end{equation*}
%where $H(\Re)$ is the entropy of set $\Re$.
where $H(\cdot)$ is the empirical entropy of $\cdot$, $\bar {\mathbb{R}}_{k-1}$ stands for  $\bar {\mathbb{R}}_{l_{k_1}^{+/-}l_{k_2}^{+/-}\cdots l_{k_{i-1}}^{+/-}}$ and $\bar {\mathbb{R}}_{k}^+$ and $\bar {\mathbb{R}}_{k}^-$ represent $\bar {\mathbb{R}}_{l_{k_1}^{+/-}\cdots l_{k_{i-1}}^{+/-}l_{k_i}^{+}}$ and $\bar {\mathbb{R}}_{l_{k_1}^{+/-}\cdots l_{k_{i-1}}^{+/-}l_{k_i}^{-}}$ respectively.

In order to get more information after each question, we employ the Iterative Dichotomiser 3 (ID3) algorithm~\cite{quinlan1986induction}, which recursively selects the question with the largest information strength as the next question, to build $\mathcal{T}$.
The algorithm can be mainly divided into four steps.
1) Calculate the information strength of every question using the whole routes set $\bar {\mathbb{R}}$.
2) Split the routes set $\bar {\mathbb{R}}_{l_{k_1}^{+/-}l_{k_2}^{+/-}\cdots l_{k_i}^{+/-}}$ into two subsets $\bar {\mathbb{R}}_{l_{k_1}^{+/-}\cdots l_{k_i}^{+/-}l_{k_{i+1}}^{+}}$ and $\bar {\mathbb{R}}_{l_{k_1}^{+/-}\cdots l_{k_i}^{+/-}l_{k_{i+1}}^{-}}$ according to the answer of question $k_{i+1}$, which has the maximum information strength among all questions.
Here we use $\bar {\mathbb{R}}_{l_{k_1}^{+/-}\cdots l_{k_i}^{+/-} l_{k_{i+1}}^{+/-}}$ to denote the routes subset after answering questions $l_{k_1},\cdots,l_{k_i}, l_{k_{i+1}}$ and the $k_{i+1}^+$ denotes that the answer of $k_{i+1}$ is yes and $k_{i+1}^-$ denotes that the answer of $k_{i+1}$ is no.
3) make a decision node of $\mathcal{T}$ containing question $k_{i+1}$.
4) perform the above steps recursively on routes subsets $\bar {\mathbb{R}}_{l_{k_1}^{+/-}\cdots l_{k_i}^{+/-}l_{k_{i+1}}^{+}}$ and $\bar {\mathbb{R}}_{l_{k_1}^{+/-}\cdots l_{k_i}^{+/-}l_{k_{i+1}}^{-}}$ using remaining questions until all the subsets have only one route.

























==> 1 IEEE_Paper_LaTeX_Template_LETTER_V2 20130719/problemdefinition.tex <==



\section{Problem Statement}\label{sec:problem}
In this section, we present some preliminary concepts and give an overview of the CrowdPlanner system. Table~\ref{tb:notation} summarized the major notations used in the rest of the paper.


\begin{table}[htb]

\caption{Summarize of notations}\label{tb:notation}
\centering\small

\begin{tabular}{|l|l|}
\hline 
{\bf \centering Notation} & {\bf \centering Definition}\tabularnewline
\hline 
$R$ & a recommended route \tabularnewline
\hline 
$\mathbb{R} $ & candidate set of recommended routes\tabularnewline
\hline 
$p$ & a place in the space\tabularnewline
\hline 
$l$ & a landmark in the space\tabularnewline
\hline 
$l.s$ & significance of landmark $l$ \tabularnewline
\hline 
$\mathbb{L}$ & a landmarks set\tabularnewline
\hline 
$\mathbb{L}_{\mathbb{R}} $ & the questioned landmark set of routes set $\mathbb{R}$ \tabularnewline
\hline 
%$p.t$ & time stamp of $p$\tabularnewline
%\hline
%$\overrightarrow{p}$ & the moving direction of $p$\tabularnewline
%\hline
%$\varphi (\overrightarrow{p_i}, \overrightarrow{p_j})$ & the angle between $\overrightarrow{p_i}$ and $\overrightarrow{p_j}$\tabularnewline
%\hline 
%$T(a_i\rightarrow a_j)$ & a trajectory travelling from $a_i$ to $a_j$\tabularnewline
%\hline 
$d(l_i,l_j)$ & Euclidean distance between landmarks $l_i$ and $l_j$\tabularnewline
\hline 
$w$ & a worker of the system\tabularnewline
\hline 
$\mathbb{W}_{\mathbb{R}}$& the selected workers of routes set $\mathbb{R}$\tabularnewline
\hline 
%$ts(a_i,a_j)$ & the timespan of object moving from $a_i$ to $a_j$\tabularnewline
%\hline
%$ts(T)$ & the timespan of  a trajectory\tabularnewline
%\hline 
%$S({*})$ & set of {$*$}\tabularnewline
%\hline 
%$|S({*})$| & the size of set $S({*})$\tabularnewline
%\hline 
\end{tabular}
\end{table}



\subsection{Preliminary Concepts}

\begin{definition}{Route:} 
A route $R$ is a continuous travelling path. 
We use a sequence $[p_1, p_2, \cdots, p_n]$, which consists of a source, a destination, and a sequence of consecutive road intersections in-between, to represent a route. 
\end{definition}


\begin{definition}{Landmark:}
A landmark is a geographical object in the space, which is stable and independent of the recommended routes. A landmark can be either a point (i.e., Point Of Interest), a line (i.e., street and high way) or a region (i.e., block and suburb) in the space.
\end{definition}



\begin{definition}{Landmark-based Route:}
A landmark-based route $\bar R$ is a route represented as a finite sequence of landmarks, i.e., $\bar R = \{l_1,l_2,...,l_n\}$.
\end{definition}

In order to obtain the landmark-based route from a raw route, we employ our previous research results on anchor-based trajectory calibration~\cite{su2013calibrating} to rewrite the continuous recommend routes into landmark-based routes, by treating landmarks as anchor points.


%For candidate routes set $\bar{ \mathbb{R}}$, we assume any two routes $\bar R_i$ and $\bar R_j$ of $\bar{\mathbb{R}}$ contain different landmarks, since in route recommendation scenario, it hardly happens that two routes connecting the same start and destination pass all the same landmarks. %$$ it might happen that two routes $R_1$ and $R_2$
%Base on the assumption, $\bar R$ also can represent the set of landmarks on it, so all the operations of set are available for $\bar R$. 


%{\bf define some operation?}
%In order to select the most significant landmark set $S$, we first need to find out which landmarks each route passes, which in other words is rewriting routes using landmarks.
%Two types of recommendation routes:
%1. \em{Google Recommendation Route}:
%A Google recommendation route is a traveling route from one place to another suggested by Google Map;
%2. \em{Historical Recommendation Route}:
%A historical recommendation route is a traveling route from one place to another generated from historical trajectories using some trajectory frequent mining algorithms.
%\subsection{ Rewriting Route}
%The current candidate routes are represented by discrete road intersections, just like Figure ? shows, that route $A$ is represented by $[t_1, t_2, t_4]$.
%In order to select the most significant landmark set $S$, we first need to find out which landmarks each route passes, which in other words is rewriting routes using landmarks.
%After rewriting using landmarks, route $A$ should be represented by $[l_1, l_2, l_3]$.
%%The route rewriting should keep the shape of the original route and connect all the passing by landmarks.
%We can adopt the Model-based Calibration method of ?, which rewrite sample-based trajectories into anchor-based trajectories, to rewrite the road-intersection-based routes into landmark-based routes, that the method can keep the shape of the original route and connect all the passing by landmarks.


\begin{definition}{Discriminative landmarks:}
A landmark set $\mathbb{L}$ is called {\em discriminative} to a set of landmark-based routes $\bar {\mathbb{R}}$ if for any two routes $\bar R_1$ and $\bar R_2$ of $\bar {\mathbb{R}}$, the joint sets $\bar {R_1} \cap \mathbb{L}$ and $\bar  {R_2}\cap \mathbb{L}$ are different.
%A route $R$ is a finite sequence of landmarks, i.e., $R = [l_1,l_2,...,l_n]$.
\end{definition}
%First, the selected landmark set $\mathbb{L}_{\mathbb{R}}$ should uniquely identify the candidate routes $\mathbb{R}$, that is for each landmark-based candidate route $\overline r$, the join set $\overline r \cap \Omega $ should be different from any other candidate routes.

For example, $\mathbb{L}_1 =\{l_3, l_4\}$ is discriminative to $ {R_1}=\{l_1, l_2, l_3\}$ and ${R_2}=\{l_1, l_2, l_4\}$, since the joint sets  $ {R_1}\cap \mathbb{L}_1=\{l_3\}$ and $ {R_2}\cap \mathbb{L}_1=\{l_4\}$ are different, but $\mathbb{L}_2 =\{l_1, l_2\}$ is not discriminative to $R_1$ and $R_2$. 

\begin{definition}{Simplest Discriminative:}
An identifiable set $\mathbb{L}$ to $\bar {\mathbb{R}}$ is simplest discriminative to $\bar {\mathbb{R}}$ if removing any landmark from $\mathbb{L}$, $\mathbb{L}$ is not discriminative to $\bar {\mathbb{R}}$ any more.
\label{define:SimplestIdentifiable}
%A route $R$ is a finite sequence of landmarks, i.e., $R = [l_1,l_2,...,l_n]$.
\end{definition}
Continuing with the previous example, $\mathbb{L}_1$ is not simplest identifiable to $\bar {\mathbb{R}}$, since after removing $l_3$ from $\mathbb{L}_1$ it still identifiable to $\bar {\mathbb{R}}$, while sets $\mathbb{L}_3=\{l_3\}$ and $\mathbb{L}_4=\{l_4\}$ are. 

%\begin{definition}{Simplest Identifiable:}
%An identifiable set $\mathbb{L}$ to $\bar {\mathbb{R}}$ is simplest identifiable to $\bar {\mathbb{R}}$ if removing any landmark from $\mathbb{L}$, $\mathbb{L}$ is not identifiable to $\bar {\mathbb{R}}$ any more.
%\label{define:SimplestIdentifiable}
%%A route $R$ is a finite sequence of landmarks, i.e., $R = [l_1,l_2,...,l_n]$.
%\end{definition}
%Continuing with the previous example, $\mathbb{L}_1$ is not simplest identifiable to $\bar {\mathbb{R}}$, since after removing $l_3$ from $\mathbb{L}_1$ it still identifiable to $\bar {\mathbb{R}}$, while sets $\mathbb{L}_3=\{l_3\}$ and $\mathbb{L}_4=\{l_4\}$ are.  

%\begin{definition}{Truth Route}
%A truth route is the best recommended routes from place $p_1$ to $p_2$ during a specific time period $t$, denoted by $T_{p_1 \rightarrow p_2}^t$. 
%\end{definition}


%\subsection{Aim of CrowdPlanner}




\subsection{Overview of CrowdPlanner}

CrowdPlanner is a two-layer system (mobile client layer and server layer) which receives user's request from mobile client specifying the source and destination, processes the request on the server and finally returns the verified best routes to the user. 
%CrowdPlanner firstly evaluates the routes recommended by web services and popular routes mined from several algorithms with the knowledge in-hand; 
%if a confidential enough evaluation cannot be made, then it will involve the human power by publishing route recommendation tasks to well experienced people to evaluate routes artificially. 
Fig.~\ref{fig:structure} shows the overview of the proposed CrowdPlanner system, which comprises two modules: traditional route recommendation (TR) and crowd-based route recommendation (CR).
The workflow of CrowdPlanner is as follows: the TR module firstly processes user's request by trying to evaluating the quality of candidate routes obtained from external sources such as map services and historical trajectory mining;
the CR module will generate a crowdsourcing task when the TR module can not distinguish the quality of candidate routes, and return the best route based on the feedbacks of human workers of the system. 

\begin{figure}
\centering
	{\psfig{figure=fig/structure.pdf,width=80mm} }
	\caption{System Overview}
	\label{fig:structure}
\end{figure}





%The traditional route recommendation module of CrowdPlanner is shown on the left side of the figure.
%It incorporates several traditional route recommendation manners, i.e., provided by web services and mined from historical trajectories. %several well used route recommendation algorithms.
%We add the `control logic' component to extend it to cope with the crowd route evaluating module which publishes evaluating tasks to target crowd workers, shown on the right side of the figure.
%We will detail the discussion for each part and their process logical in the subsequent section.

%\begin{figure}
%\centering
%	{\psfig{figure=fig/logical.jpg,width=68.7mm} }
%	\caption{logical}
%	\label{fig:logical}
%\end{figure}

\subsubsection{Traditional Route Recommendation Module}
%Just as the Fig.~\ref{fig:askquestion} shown, when a client user submits a recommendation request, which specifies he wants to go to the best recommended routes from `Nanjing Confucius Temple' to `Nanjing Railway Station' fifteen minutes later and he awards the request for five coins (the virtual currency of CrowdPlanner), the {\em control logic component} of the traditional route evaluating module handles it.
%\begin{figure}[h]
%\centering
%	{\psfig{figure=fig/askquestion.png,width=35mm} }
%	\caption{Distinguishable landmarks of any two routes}
%	\label{fig:askquestion}
%\end{figure}

This module processes the user's request by generating a set of candidate routes from external sources (route generation component) and evaluating the quality of those routes automatically without involving human effort (route evaluation component). 

{\bf Control logic component:} 
This component receives the user's request and controls the workflow of the entire system. It also coordinates the interactions between the TR module and CR module. 
Once a user's request is received by the control logic component, it will invoke {\em reuse truth component} to match the request to the verified routes (truth) between two places at his departure time. 
If the new coming request is a hit of the truth, the system will return result immediately.
Otherwise the component will invoke the {\em route generation component} to automatically generate some candidate routes and {\em route evaluation component} to evaluate the qualities of these candidate routes using the verified truth.

%{\bf Cache component:} Cache component caches the recent query results into main memory.
%If the new coming query is a hit of the cache, the cache component will return result immediately.
%Otherwise it will invoke the {\em route generating component} to automatically generate some candidate routes.


{\bf Route evaluation component:} 
This component evaluates the routes using computer power and it provides an efficient way to reduce the cost of CrowdPlanner, since it can largely reduce the amount of tasks generated.
The component will firstly build up a candidate route set by invoking {\em route generation component}. 
%the candidate routes provided by web services and mined popular routes by 
If some of these routes agree with each other to a high degree, one of them will be selected as the best recommended route and added into a truth database with the corresponding time tag. 
If a best recommended route can not be determined, the system will assign each candidate route a confidence score, which is generated by the verified truths and illustrates the possibility of the route to be the best recommended route.
%The score . 
A route with the highest confidence score that is greater than a threshold $\eta$ will be regarded to be the best recommended and returned to the user; % the best route; 
%otherwise there is no verified best route ensured.
%If there is a route which is the , the system will return the best route with its confidence; 
otherwise the logic control will hand over the request to the CR module.
%The details of the evaluating using verified will be presented in Sec.~\ref{sec:truthreuse}.

%If the distance between the two types of candidate routes is less than a threshold $\eta_{comp}$, or if the occurrence of the historical term of candidates answer is not less than a threshold $\eta_k$, then we treat the historical term of candidates route as the query result, then we return it and insert the best route between two certain locations into truth.
%Otherwise the compare component will invoke the {\em truth reusing component} to evaluate these candidate routes and judge which route is the best.


{\bf Route generation component:} This component generates two types of candidate routes, the one provide by web services such as Google Map and the one generated from historical trajectories by using popular route mining algorithms, i.e., MPR, LDR and MFP.


%{\bf Truth reusing component:} The truth reusing component can evaluate the candidate answers %using the existing truth
%if some existing truths can be used be matched to the candidate answers.
%If not, the CrowdPlanner will invoke the crowd route recommend module to publish a Crowdsourcing task.
%It provides a efficient way to reduce the cost of CrowdPlanner, since it can largely reduce the amount of Crowding tasks.
%The details of the truth reusing component will be presented in Sec.~\ref{sec:truthreuse}.

\subsubsection{Crowd Route Recommendation Module}
Crowd route recommendation module will take over the route recommendation request when the traditional route recommendation module cannot provide the best route with high enough confidence.
The module will generate a crowdsourcing task consisting of a series simple but informative binary questions (task generation component), and assign the task to a set of selected worker who are most suitable to answer these questions (worker selection component).

{\bf Task generation component:} 
As the core of CrowdPlanner, this component generates a task by proposing a series of questions for workers to answer. It is beneficial to have these questions as simple and compact as possible, since both the accuracy and economic effectiveness of the system can be improved. The design of this component will address two important issues: {\em what to ask in questions} and {\em how to ask the questions}. We will discuss the detailed mechanism of this part in Section~\ref{sec:generatequestion}.

{\bf Worker selection component:} 
This is another core component of CrowdPlanner. 
In order to maximize the effectiveness of the system, we need to select a set of eligible workers who are most suitable to answer the questions in a given task, by estimating the worker's familiarity with the area of request. Technical details of this component will be presented in Section~\ref{sec:targetworker}. 

{\bf Early stop component:} 
In most cases, we do not to need to wait for all the answers of the assigned workers.
When partial feedbacks have been collected, this component will evaluate the confidence of the answer and return the result to the user as early as possible when the confidence is high enough. 
%Sec.~\ref{sec:earlystop} will detail how the early stop algorithm works.


{\bf Rewarding component:}
This component rewards the workers according to their workload and the quality of their answers. The reward points can be used later when they request a route recommendation in CrowdPlanner. 

\vspace{1em}
In the following two sections, we will present the design and technical details of the two core components of CrowdPlanner: task generation and worker selection. 


==> 1 IEEE_Paper_LaTeX_Template_LETTER_V2 20130719/relatedwork.tex <==
\section{Related Work}\label{sec:related}
To our knowledge, there is no existing work on evaluating the quality of recommended routes. % trajectory calibration or trajectory rewriting. 
As the goal of this work is to evaluate the quality of recommended routes by web services and mining algorithms, the route recommendation algorithms (mining frequent path algorithms) used in this paper are reviewed first. 
% improve the effectiveness of similarity-based analysis, the distance measures studied in this paper are also reviewed at last.
Then we will review route generating algorithms.
Since in our Crowdplanner system, we reuse truth to reduce the request times of Crowdsourcing, which share similar inspiration and techniques with route generating.
Also we leverage the generating easy questions and  finding target workers to improve the quality of evaluating and reduce the workers' workload, which share the same motivation of some research works of Crowdsourcing question designing and workers selecting.  
Therefore in the last of this section, we will review these two lines of related work. 
%Our work aims to format trajectories which can be regarded as reducing the uncertainty of trajectories. 
%We need apply trajectory complementing by inserting points highly likely to be on the trajectory, that is related to find popular route. 
%The calibration can improve the accuracy of trajectory distance measures,
% after mapping trajectory into reference system.

{\bf Route Recommendation Algorithms.}
The popular routes mining has received tremendous research interests for a decade and a lot of works are on it, such as \cite{sacharidis2008line, mamoulis2004mining, giannotti2007trajectory, gonzalez2007adaptive, zheng2009mining,giannotti2007trajectory, mamoulis2004mining,gonzalez2007adaptive,zheng2009mining,li2007traffic,lee2007trajectory,gaffney1999trajectory,lee2008traclass}.
%investigates efficient ways to find and monitor popular motion paths that are defined as those visited by a certain number of moving objects, but it is limited to mine frequently visited paths only. 
%The focus of
%\cite{mamoulis2004mining, giannotti2007trajectory, gonzalez2007adaptive, zheng2009mining}
% is on mining trajectory patterns to help find the popular routes from a start location to a destination.
%\cite{giannotti2007trajectory}
% proposes to mine a sequence of temporally annotated points called T-pattern, in order to
% find all T-patterns with sufficiently high support.
%Similarly, in \cite{mamoulis2004mining,gonzalez2007adaptive,zheng2009mining}, frequent paths or sequences are explored by existing sequential pattern mining algorithms.
Among these works, \cite{chen2011discovering, wei2012constructing,Luo2013Finding, Ceikut2013Routing} are the most representative.   
Chen et al. \cite{chen2011discovering} proposes a novel popularity function for
path desirability evaluation using historical
trajectory datasets. 
The popular routes recommended by it tends to have fewer vertices. 
%Here we propose both linear complement and model-based complement methods to recovery the trajectory from a start point to a destination. 
%Linear complementing is easy and straightforward;
%model-based complementing finds very popular visited point between two given points and gives these points' existing probability considering both forward and backward probability.
The work in~\cite{wei2012constructing} provides k popular routes by mining uncertain trajectories. 
The recommendation routes of this work tend to be rough routes instead of correct routes. 
%Assuming that there is no map at hand, they focus on how to derive rough routes from the uncertain trajectory data. 
\cite{Luo2013Finding} claims the popular routes change as time, so it carries out a popular routes mining algorithms which can provide the recommended routes in arbitrary time periods specified by the users. 
\cite{Ceikut2013Routing} provides the evidences that the routes recommended by web services are sometimes different from drivers' preference. 
Thus it mines the individual popular routes from his historical trajectories. 
The recommended routes of this method reflect certain people's preference. %same observation


{\bf Question Designing.}
Question designing is always an application dependent strategy, which may consider the cost of questions or the number of questions. 
\cite{guo2012so, parameswaran2012crowdscreen} propose strategies to minimize the cost of the questions designed.
The question designing strategy of~\cite{wang2012crowder} is to minimize the number of questions. 
The question designing strategy of~\cite{parameswaran2011human} is to generate the optimal set of questions. 
%Researcher have Works have addressed the issue. 


{\bf Worker Selecting.}
Selecting workers with high individual qualities for tasks always does beneficial to the final quality of answers. 
Thus~\cite{lappas2009finding} propose an algorithm to select workers fulfilling some skills with the minimized the cost of choosing them. 
In~\cite{campbell2003expertise} use emails communication to identifying skillful workers. %identification.
Cao et al~\cite{cao2012whom} assign tasks to micro-blog users by mining users' knowledge and measuring their error rate. 



 













